Error Cancellation in Diffusion Monte Carlo Calculations of Surface Chemistry

Diffusion Monte Carlo (DMC) is being recognized as a higher-accuracy, albeit more computationally expensive, alternative to Density Functional Theory (DFT) for energy predictions of catalytic systems. A major computational bottleneck in the use of DMC for catalysis is the need to perform finite-size extrapolations by simulating increasingly large periodic cells (supercells) to eliminate many-body finite-size effects and obtain energies in the thermodynamic limit. Here, we show that this computational cost can be significantly reduced by leveraging the cancellation of many-body finite-size errors that accompanies the evaluation of energy differences when calculating quantities like binding energies and mapping potential energy surfaces. We test the error cancellation and convergence in two well-known adsorbate/slab systems, H2O/LiH(001) and CO/Pt(111). Based on this, we identify strategies for obtaining binding energies in the thermodynamic limit that optimize error cancellation to balance accuracy and computational efficiency. We then predict the correct order of adsorption site preference on CO/Pt(111), a challenging problem for DFT. Our accurate, inexpensive DMC calculations recover the top > bridge > hollow site order, in agreement with experimental observations. We proceed to map the potential energy surface of CO hopping between Pt(111) adsorption sites. This reveals the existence of an L-shaped top-bridge-hollow diffusion trajectory characterized by energy barriers that provide an additional kinetic justification for experimental observations of CO/Pt(111) adsorption. Overall, this work demonstrates that it is routinely possible to achieve order-of-magnitude speedups and memory savings in DMC calculations by taking advantage of error cancellation in the calculation of energy differences that are ubiquitous in heterogeneous catalysis and surface chemistry more broadly.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
